Tightly-coupled Visual-DVL-Inertial Odometry for Robot-based Ice-water Boundary Exploration

Robotic underwater systems, e.g., Autonomous Underwater Vehicles (AUVs) and Remotely Operated Vehicles (ROVs), are promising tools for collecting biogeochemical data at the ice-water interface for scientific advancements. However, state estimation, i.e., localization, is a well-known problem for robotic systems, especially, for the ones that travel underwater. In this paper, we present a tightly-coupled multi-sensors fusion framework to increase localization accuracy that is robust to sensor failure. Visual images, Doppler Velocity Log (DVL), Inertial Measurement Unit (IMU) and Pressure sensor are integrated into the state-of-art Multi-State Constraint Kalman Filter (MSCKF) for state estimation. Besides that a new keyframe-based state clone mechanism and a new DVL-aided feature enhancement are presented to further improve the localization performance. The proposed method is validated with a data set collected in the field under frozen ice, and the result is compared with 6 other different sensor fusion setups. Overall, the result with the keyframe enabled and DVL-aided feature enhancement yields the best performance with a Root-mean-square error of less than 2 m compared to the ground truth path with a total traveling distance of about 200 m.

==> 0_macros.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%% Customized packages and settings (start) %%%%%%%%%%%%%%%%%%

%%%% Customized Packages %%%%
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{lipsum} % Just for generating dummy text, can be removed
\usepackage{gensymb} % for \degree
\usepackage{xparse}

%%%% Reference Commands %%%%
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\Eref}[1]{Equation~\eqref{#1}}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}


%%%% Tricks for Compact Layout %%%%
% Caption configuration 
\usepackage[labelsep=period]{caption}
\captionsetup{font=small}
\captionsetup[table]{aboveskip=3pt}
\captionsetup[table]{belowskip=2pt}
\captionsetup[figure]{aboveskip=5pt}
\captionsetup[figure]{belowskip=0pt}

% Reduce the margin before paragraph
\renewcommand{\paragraph}[1]{\vspace{0.2em}\noindent \textbf{#1 \hspace{0.2em}}}




%%%% Macors %%%%

% Author comments
\newcommand{\gy}[1]{\textcolor{magenta}{{[GY: #1]}}}
\newcommand{\todo}[1]{\textcolor{MyDarkRed}{{[TODO: #1]}}}

% Just for tutorial
\definecolor{MyDarkRed}{rgb}{0.66, 0.16, 0.16}
\definecolor{MyDarkBlue}{rgb}{0.16, 0.16, 0.66}
\newcommand{\dummycolor}{lightgray} 
\newcommand{\correct}[1]{\textcolor{MyDarkBlue}{#1 \checkmark}}
\newcommand{\wrong}[1]{\textcolor{MyDarkRed}{#1 $\times$}}

% Variable abbreviations
\newcommand{\MethodName}{AGreatDeepNet\xspace}

% Math notations
\newcommand{\energy}{E}
\newcommand{\mass}{m}
\newcommand{\speedoflight}{c}

%%%%%%%%%%%%%%%%%% Customized packages and settings (end) %%%%%%%%%%%%%%%%%%



==> 9_acknowlegment.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                         Acknowlegment                                %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Acknowlegment}
\label{sec:acknowlegment}

This work is supported by NSF XXXX and URI
[same sentences can be found in our oceans paper]
